Vertical-Horizontal Structured Attention for Generating Music with Chords

In this paper, we propose a lightweight music-generating model based on variational autoencoder (VAE) with structured attention. Generating music is different from generating text because the melodies with chords give listeners distinguished polyphonic feelings. In a piece of music, a chord consisting of multiple notes comes from either the mixture of multiple instruments or the combination of multiple keys of a single instrument. We focus our study on the latter. Our model captures not only the temporal relations along time but the structure relations between keys. Experimental results show that our model has a better performance than baseline MusicVAE in capturing notes in a chord. Besides, our method accords with music theory since it maintains the configuration of the circle of fifths, distinguishes major and minor keys from interval vectors, and manifests meaningful structures between music phrases.

==> chapters/_algorithm.tex <==
\section{Algorithm}
\subsection{$\alpha-\beta-\gamma$ channels for Social Relation Inference}
Three inference processes are identified for each relation edge $e_{ij}$: the $\alpha(D)$ process detects relation $e_{ij}$ directly from dialogue features, the $\beta(e_{ij})$ process predicts $v_i$ and $v_j$ from $e_{ij}$, and the $\gamma(v_i,v_j)$ computes $e_{ij}$ by binding its connected nodes $v_i$ and $v_j$. Through recursively repeating this process, we could reason about social relation from available information.

We rewrite the posterior in the problem formulation with Bayes' theorem and Gibbs distribution:
\begin{equation}
    \begin{aligned}
    p(pg|D;\theta) &\propto P(D|pg;\theta)P(pg;\theta) \\
                   &=\frac{1}{Z} exp \{-\mathcal{E}(D|pg;\theta) -\mathcal{E}(pg;\theta)\}
    \end{aligned}
\end{equation}
$Z$ is the normalization constant. Define the dialog as a sequence of words: $D=\{w_1,w_2,...,w_n\}$, then the likelihood can be expressed as:
\begin{equation}
    \begin{aligned}
    p(D|pg) &= \prod_{t=1}^{T} P(w_t|\mathbf{c_t},pg) \\
            &=\prod_{t=1}^{T}P(w_t|\mathbf{c_t})\cdot P(w_t|pg)
    \end{aligned}
\end{equation}
, where context vector $\mathbf{c_t}=[w_1,...,w_{t-1},w_{t+1},...,w_n]$, and we assume $\mathbf{c_t}$ and $pg$ are conditionally independent given $w_t$. Similarly, $P(w_t|pg)$ can be expressed as: 
\begin{equation}
    P(w_t|pg) = \prod_{\mathbf{v_i}\in V(pg)}P(w_t|\mathbf{v_i})\cdot\prod_{\mathbf{e_{ij}}\in E(pg)}P(w_t|\mathbf{e_{ij}})\}.
\end{equation}
Intuitively, the word selection either depends on its word context $P(w_t|\mathbf{c_t})$ or the personal attributes $P(w_t|\mathbf{v_i})$ or the social relation $P(w_t|\mathbf{e_{ij}})$. $P(w_t|\mathbf{c_t})$ is given by a language model and $P(w_t|\mathbf{v_i})$ and $P(w_t|\mathbf{e_{ij}})$ are estimated from word selection frequency with Maximum Likelihood Estimation (MLE).
We can thus define the following energy terms:
\begin{equation}
    \begin{aligned}
    \mathcal{E}(D|pg;\theta) =& \sum_{t=1}^{T}(\mathcal{E}(w_t|c_t) + \sum_{v_i}\mathcal{E}(w_t|v_i) + \sum_{e_{ij}}\mathcal{E}(w_t|e_{ij})) \\ 
                             =&-\sum_{t=1}^{T}\{log(P(w_t|c_t)) + \sum_{v_i} \alpha_i\log(p(w_t|v_i)) \\
                              &+\sum_{e_{ij}} \alpha_{ij}\log(p(w_t|e_{ij}))\}
    \end{aligned}
\end{equation}
We can use language model $F$ to score the sentence: 
\begin{equation}
    \begin{aligned}
    \sum_{t=1}^{T}log(P(w_t|c_t))=\alpha\sum_{t=1}^{T}F_i(D)
    \end{aligned}
\end{equation}
The parse graph prior can be written as:
\begin{equation}
    \begin{aligned}
    \mathcal{E}(pg;\theta) = &-\sum_{e_{ij}\in E(D^{(t)})} \beta_i\log(p(v_i|e_{ij})) \\
                             &-\sum_{e_{ij}\in E(D^{(t)})} \beta_j\log(p(v_j|e_{ij})) \\
                             &-\sum_{v_i,v_j\in V(D^{(t)})} \gamma_{ij}\log(p(e_{ij}|v_i,v_j))
    \end{aligned}
\end{equation}
Combine equation (5), (8) (9) and (10), the posterior can be formulated as:
\begin{equation}
    \begin{aligned}
    p(pg|D;\theta) \propto   &\alpha\sum_{t=1}^{T}F_i(D) + \sum_{v_i} \alpha_i\log(p(w_t|v_i)) \\
                             &+\sum_{e_{ij}} \alpha_{ij}\log(p(w_t|e_{ij}))\} \\
                             &+\sum_{e_{ij}\in E(D^{(t)})} \beta_i\log(p(v_i|e_{ij})) \\
                             &+\sum_{e_{ij}\in E(D^{(t)})} \beta_j\log(p(v_j|e_{ij})) \\
                             &+\sum_{v_i,v_j\in V(D^{(t)})} \gamma_{ij}\log(p(e_{ij}|v_i,v_j))
    \end{aligned}
\end{equation}

\textbf{$\alpha$ channel}: We estimate the social relation and attributes directly from the dialogue data.

\textbf{$\beta$ channel}: Then, we use the relation edge $e_{ij}$ to update the attributes of node $v_i$ and $v_j$.

\textbf{$\gamma$ channel}: Reversely, we use the attributes of node $v_i$ and $v_j$ to update the relation edge $e_{ij}$.

By iteratively repeating the $\alpha-\beta-\gamma$ process, we continuously take in the information from the dialogue based on a discriminative model. Then we reason about people's pairwise relationship from their attributes. We also infer people's personal attributes from their relationships. 

\subsection{Incremental Beyesian Inference}
Since the personal attributes and social relations are constrained by multiple energy terms, we utilize a Markov chain Monte Carlo (MCMC) sampler to update our parse graph belief from the posterior in the last section. We start from a default social relation $pg^{(0)}$ and prior distribution $P(pg^{(0)};\theta)$ during initialization. A new sample $pg^{(t)}$ will be updated from $pg^{(t-1)}$ after the Markov chain converges. We design two types of Markov chain dynamics which are used at random probabilities $q_i, i=1,2$ to make proposal moves:
\begin{itemize}
\item Dynamics $q_1$: flip of the attributes $v_i$. 
\item Dynamics $q_2$: flip of the social relation $e_{ij}$.
\end{itemize}
Using the Metropolis-Hastings algorithm, the proposed new parse graph $pg'$ is accepted according to the following acceptance probability:
\begin{equation}
    \begin{aligned}
    \alpha(pg'|pg, D;\theta) &=\min(1, \frac{P(pg'|D;\theta)P(pg|pg')}{P(pg|D;\theta)P(pg'|pg)}) \\
                             &=\min(1, \frac{P(pg'|D;\theta)}{P(pg|D;\theta)})
    \end{aligned}
\end{equation}
where the proposal probability rate is cancelled out since the proposal moves are symmetric in probability. 

